Design Space Exploration of Sparsity-Aware Application-Specific Spiking Neural Network Accelerators

Spiking Neural Networks (SNNs) offer a promising alternative to Artificial Neural Networks (ANNs) for deep learning applications, particularly in resource-constrained systems. This is largely due to their inherent sparsity, influenced by factors such as the input dataset, the length of the spike train, and the network topology. While a few prior works have demonstrated the advantages of incorporating sparsity into the hardware design, especially in terms of reducing energy consumption, the impact on hardware resources has not yet been explored. This is where design space exploration (DSE) becomes crucial, as it allows for the optimization of hardware performance by tailoring both the hardware and model parameters to suit specific application needs. However, DSE can be extremely challenging given the potentially large design space and the interplay of hardware architecture design choices and application-specific model parameters. In this paper, we propose a flexible hardware design that leverages the sparsity of SNNs to identify highly efficient, application-specific accelerator designs. We develop a high-level, cycle-accurate simulation framework for this hardware and demonstrate the framework's benefits in enabling detailed and fine-grained exploration of SNN design choices, such as the layer-wise logical-to-hardware ratio (LHR). Our experimental results show that our design can (i) achieve up to $76\%$ reduction in hardware resources and (ii) deliver a speed increase of up to $31.25\times$, while requiring $27\%$ fewer hardware resources compared to sparsity-oblivious designs. We further showcase the robustness of our framework by varying spike train lengths with different neuron population sizes to find the optimal trade-off points between accuracy and hardware latency.

==> figures/garbage.tex <==
\begin{table*}[t]
\centering
    \begin{tabular}{|c||c|c|c|c|c|c|}
        \hline
         & & &  \textbf{BRAM} & \textbf{Clock} & \textbf{BRAM - Lat.} & \textbf{BRAM} \\
        \textbf{Dataset} & S_{l1}/S_{l2}/S_{l3} & (U_{l1}, U_{l2}, U_{l3}) & \textbf{Blocks} & \textbf{Cycles} & \textbf{Impr.} & \textbf{Util.} \\
            \hline \hline
            \multirow{8}{*}{MNIST}  & \multirow{8}{*}{107/75/24}     
            & (1, 1, 1) & 900 & 7052 & --- & 67\%\\
            && (2, 1, 1) & 750 & 9996 & $\times$0.833, $\times$1.41 & 56\% \\
            && (1, 2, 1) & 750 & 10044 & $\times$0.833, $\times$1.42 & 56\% \\
            && (1, 1, 2) & 750 & 7562 & $\times$0.833, $\times$1.07 & 56\% \\
            && (2, 2, 4) & 375 & 12428 & $\times$0.413, $\times$1.76 & 28\% \\
            && (4, 2, 4) & 300 & 18040 & $\times$0.332, $\times$2.55 & 22\% \\
            && (4, 8, 8) & 150 & 24568 & $\times$0.166, $\times$3.48 & 11\% \\
            && (4, 8, 16) & 132 & 25248 & $\times$0.146, $\times$3.54 & 11\% \\
            \hline
            \multirow{10}{*}{FMNIST} & \multirow{10}{*}{217/58/60} 
            & (1, 1, 1) & 900 & 11676 & --- & 67\%\\
            && (2, 1, 1) & 750 & 18423 & $\times$0.833, $\times$1.58 & 56\% \\
            && (1, 2, 1) & 750 & 11845 & $\times$0.833, $\times$1.01 & 56\% \\
            && (1, 1, 2) & 750 & 11814 & $\times$0.833, $\times$1.01 & 56\% \\
            && (2, 2, 4) & 375 & 19167 & $\times$0.413, $\times$1.64 & 28\% \\
            && (2, 4, 8) & 262 & 21346 & $\times$0.291, $\times$1.83 & 19\% \\
            && (4, 2, 4) & 300 & 33553 & $\times$0.332, $\times$2.88 & 22\% \\
            && (4, 8, 8) & 150 & 36571 & $\times$0.166, $\times$3.14 & 11\% \\
            && (4, 8, 16) & 132 & 41156 & $\times$0.146, $\times$3.58 & 11\% \\
            && (2, 8, 4) & 262 & 20834 & $\times$0.291, $\times$1.79 & 19\% \\
            \hline
    \end{tabular}
    \caption{Layer-wise memory unit size vs latency results. Column $S$ represents input spike count for its associated layer, and column $U$ represents memory unit size. Network topology used for both MNIST and FMNIST: $784\times300\times300\times300$ with population coding and spike train length of 8, accuracy is 80.1\% for FMNIST and 93.5 for for MNIST. The BRAM utilization results are for XCVU37P-L2FSVH2892E FPGA}
    \label{tab:mem_config}
 \end{table*}


 \begin{table*}[t]
\centering
    \begin{tabular}{|c||c|c|c|c|c|c|c|}
        \hline
         & \textbf{Network} & & \textbf{Mapping} & \textbf{Area Estimation} & \textbf{Clock} & \textbf{LUT - Lat.} & \textbf{Acc} \\
        \textbf{Dataset} & \textbf{Topology} & \textbf{Work} & \textbf{Ratio} & \textbf{LUT / REG / BRAM} & \textbf{Cycles} & \textbf{Impr.} & \% \\
            \hline \hline
            \multirow{6}{*}{MNIST} & \multirow{6}{*}{784-1024-}    
            & Ju et. al.\cite{abderrahmane2020design} & 1-1-1 & 67.8K/45.3K/900 & 7052 & --- & 67\%\\
            && This Work & 1-1-1 & 67.8K/45.3K/900 & 9996 & $\times$0.833, $\times$1.41 & 56\% \\
            && This Work & 1-1-1 & 67.8K/45.3K/900 & 10044 & $\times$0.833, $\times$1.42 & 56\% \\
            &1024-10& \textbf{TW}^{(1, 2, 1)} & 1-1-1 & 67.8K/45.3K/900 & 7562 & $\times$0.833, $\times$1.07 & 56\% \\
            &(MLP)& This Work} & 1-1-1 & 67.8K/45.3K/900 & 12428 & $\times$0.413, $\times$1.76 & 28\% \\
            && This Work & 1-1-1 & 67.8K/45.3K/900 & 18040 & $\times$0.332, $\times$2.55 & 22\% \\
            \hline
            \multirow{6}{*}{FMNIST} & \multirow{4}{*}{28x28-64C5-P2-} 
            & \cite{abderrahmane2020design} & 67.8K/45.3K/900 & 7052 & --- & 67\%\\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 18423 & $\times$0.833, $\times$1.58 & 56\% \\
            &64C5-P2-128-10& \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 11845 & $\times$0.833, $\times$1.01 & 56\% \\
            &(VGG)& \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 11814 & $\times$0.833, $\times$1.01 & 56\% \\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 19167 & $\times$0.413, $\times$1.64 & 28\% \\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 20834 & $\times$0.291, $\times$1.79 & 19\% \\
            \hline
            \multirow{6}{*}{SVHN} & \multirow{4}{*}{28x28-64C5-P2-} 
            & \cite{abderrahmane2020design} & 67.8K/45.3K/900 & 7052 & --- & 67\%\\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 18423 & $\times$0.833, $\times$1.58 & 56\% \\
            &64C5-P2-128-10& \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 11845 & $\times$0.833, $\times$1.01 & 56\% \\
            &(AlexNet)& \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 11814 & $\times$0.833, $\times$1.01 & 56\% \\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 19167 & $\times$0.413, $\times$1.64 & 28\% \\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 20834 & $\times$0.291, $\times$1.79 & 19\% \\
            \hline
                        \multirow{6}{*}{CIFAR-10} & \multirow{4}{*}{28x28-64C5-P2-} 
            & \cite{abderrahmane2020design} & 67.8K/45.3K/900 & 7052 & --- & 67\%\\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 18423 & $\times$0.833, $\times$1.58 & 56\% \\
            &64C5-P2-128-10& \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 11845 & $\times$0.833, $\times$1.01 & 56\% \\
            &(AlexNet)& \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 11814 & $\times$0.833, $\times$1.01 & 56\% \\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 19167 & $\times$0.413, $\times$1.64 & 28\% \\
            && \textbf{TW}^{(2, 1, 1)} & 67.8K/45.3K/900 & 20834 & $\times$0.291, $\times$1.79 & 19\% \\
            \hline
    \end{tabular}
    \caption{Layer-wise memory unit size vs latency results. Column $S$ represents input spike count for its associated layer, and column $U$ represents memory unit size. Network topology used for both MNIST and FMNIST: $784\times300\times300\times300$ with population coding and spike train length of 8, accuracy is 80.1\% for FMNIST and 93.5 for for MNIST. The BRAM utilization results are for XCVU37P-L2FSVH2892E FPGA}
    \label{tab:mem_config}
 \end{table*}
